Populous: A tool for populating ontology templates

We present Populous, a tool for gathering content with which to populate an ontology. Domain experts need to add content, that is often repetitive in its form, but without having to tackle the underlying ontological representation. Populous presents users with a table based form in which columns are constrained to take values from particular ontologies; the user can select a concept from an ontology via its meaningful label to give a value for a given entity attribute. Populated tables are mapped to patterns that can then be used to automatically generate the ontology's content. Populous's contribution is in the knowledge gathering stage of ontology development. It separates knowledge gathering from the conceptualisation and also separates the user from the standard ontology authoring environments. As a result, Populous can allow knowledge to be gathered in a straight-forward manner that can then be used to do mass production of ontology content.

==> abstract.tex <==
\begin{abstract}
We present  \toolname, a tool for gathering content with which to populate an ontology.
Domain experts need to add content, that is often repetitive in its form, without having to tackle the underlying ontological representation.
Ontologies can be created  through patterns of axioms where a type of concept is described in terms of other concepts---the classic genus and differentiae.
These patterns or templates need to be populated by domain experts that choose concepts to form the descriptions  from existing ontologies.
\toolname presents users with a table based form in which columns are constrained to take values from particular ontologies; the user can select a concept from an ontology via its meaningful label.
these tables of semantically constrained   data are mapped to patterns that then automatically generate the ontology's contnet.
\toolname's contribution is in the knowledge gathering stage of ontology development.
It separates knowledge gathering from the conceptualisation and also separates the user from the standard ontology authoring environments.
 


\end{abstract}
